O(log log rank) Competitive-Ratio for the Matroid Secretary Problem

In the \textit{Matroid Secretary Problem} (MSP), the elements of the ground set of a Matroid are revealed on-line one by one, each together with its value. An algorithm for the MSP is \textit{Matroid-Unknown} if, at every stage of its execution: (i) it only knows the elements that have been revealed so far and their values, and (ii) it has access to an oracle for testing whether or not any subset of the elements that have been revealed so far is an independent set. An algorithm is \textit{Known-Cardinality} if, in addition to (i) and (ii), it also initially knows the cardinality of the ground set of the Matroid. We present here a Known-Cardinality and \textit{Order-Oblivious} algorithm that, with constant probability, selects an independent set of elements, whose value is at least the optimal value divided by $O(\log{\log{\rho}})$, where $\rho$ is the rank of the Matroid; that is, the algorithm has a \textit{competitive-ratio} of $O(\log{\log{\rho}})$. The best previous results for a Known-Cardinality algorithm are a competitive-ratio of $O(\log{\rho})$, by Babaioff \textit{et al.} (2007), and a competitive-ratio of $O(\sqrt{\log{\rho}})$, by Chakraborty and Lachish (2012). In many non-trivial cases the algorithm we present has a competitive-ratio that is better than the $O(\log{\log{\rho}})$. The cases in which it fails to do so are easily characterized. Understanding these cases may lead to improved algorithms for the problem or, conversely, to non-trivial lower bounds.

==> acknowledgements.tex <==
\section*{Acknowledgements}
We would like to thank Ran El-Yaniv, Eldar Fischer and Ilan Newman for useful discussions.
We would also like to thank Oren Ben-Zwi, Trevor Fenner, Sven Helmer and Alex Popa for helping in the editing and verifying the results.
